The ABC of Pair Programming: Gender-dependent Attitude, Behavior and Code of Young Learners

Young learners are increasingly introduced to programming, and one of the main challenges for educators is to achieve learning success while also creating enthusiasm. As it is particularly difficult to achieve this enthusiasm initially in young females, prior work has identified gender-specific differences in the programming behavior of young learners. Since pair programming, which turns programming into a more sociable activity, has been proposed as an approach to support programming education, in this paper we aim to investigate whether similar gender-specific characteristics can also be observed during pair programming. Therefore, we designed a gender-neutral introductory SCRATCH programming course tailored for integrating pair programming principles, and conducted it with a total of 139 students aged between 8 and 14 years. To identify gender-dependent differences and similarities, we measure the attitude towards programming and the course setting, observe the behavior of the students while programming, and analyze the code of the programs for different gender-combinations. Overall, our study demonstrates that pair programming is well suited for young learners and results in a positive attitude. While the resulting programs are similar in quality and complexity independent of gender, differences are evident when it comes to the compliance to pair programming roles, the exploration of code, and the creative customization of programs. These findings contribute to an in-depth understanding of social and technical gender specifics of pair programming, and provide educators with resources and guidance for implementing gender-sensitive pair programming in the classroom.

==> content/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

....

We know from previous research that girls tend to implement less complex programs because they prefer project types like stories, which tend to require sequences. However, our course design has shown that girls also have a lot of fun implementing a game, approaching the complexity of the young programs, and letting loose creatively. ~\cite{grassl2021}

...

==> content/tables/funDiffRanking.tex <==
\begin{table}[t]
\centering
\caption{Ranking from students' responses for each task regarding their perceived fun and difficulty in percentage.}
\label{tab:ranking}
\begin{tabular}{llrrrrrr}
\toprule
Category & Pair & 1 & 2 & 3 & 4 & 5 & 6  \\
\midrule
%\multirow[c]{3}{*}{likeTask}  & ff & 0.86 & 0.79 & 0.83 & 0.76 & 0.80 & 0.87 \\
%f-m & 0.64 & 0.75 & 0.72 & 0.71 & 0.88 & 0.75 & 0.73 \\
%& mm & 0.76 & 0.80 & 0.82 & 0.81 & 0.88 & 0.90 \\ \midrule
\multirow[c]{3}{*}{mostFun} & ff & 27.66 & 12.77 & 19.15 & 8.51 & 19.15 & 12.77  \\
% & f-m & 16.67 & 16.67 & 33.33 & 33.33 & 0.00 & 0.00  \\
 & mm & 8.33 & 13.89 & 15.28 & 12.50 & 29.17 & 20.83  \\ \midrule
\multirow[c]{3}{*}{leastFun} & ff  & 23.26 & 13.95 & 23.26 & 18.60 & 11.63 & 9.30  \\
% &  f-m & 16.67 & 16.67 & 16.67 & 0.00 & 16.67 & 33.33  \\
 & mm & 32.08 & 26.42 & 13.21 & 15.09 & 9.43 & 3.77  \\ \midrule
\multirow[c]{3}{*}{mostHard} & ff  & 6.25 & 2.08 & 22.92 & 35.42 & 18.75 & 14.58  \\
% &  f-m & 0.00 & 33.33 & 0.00 & 33.33 & 16.67 & 16.67  \\
 & mm & 10.53 & 7.02 & 22.81 & 19.30 & 15.79 & 24.56   \\ \midrule
\multirow[c]{3}{*}{mostEasy} & ff  & 75.56 & 13.33 & 2.22 & 2.22 & 4.44 & 2.22  \\
 %&  f-m & 66.67 & 16.67 & 16.67 & 0.00 & 0.00 & 0.00  \\
 & mm & 66.07 & 16.07 & 7.14 & 3.57 & 0.00 & 7.14  \\
\bottomrule
\end{tabular}
\end{table}

 
% \begin{table}[t]
%\centering
%\caption{Ranking from students survey for the tasks regarding their peceived fun and difficulty in percentage.}
%\label{tab:ranking}
%
%\begin{tabular}{ccccccccccccc}
%\toprule
%task &  & mostFun &  & leastFun &  &  &  & mostHard &  &  & leastHard &  \\ 
% & f-f & f-m & m-m & f-f & f-m & m-m & f-f & f-m & m-m & f-f & f-m & m-m \\ \midrule
%1 &  &  &  &  &  &  &  &  &  &  &  &  \\
%2 &  &  &  &  &  &  &  &  &  &  &  &  \\
%3 &  &  &  &  &  &  &  &  &  &  &  &  \\
%4 &  &  &  &  &  &  &  &  &  &  &  &  \\
%5 &  &  &  &  &  &  &  &  &  &  &  &  \\
%6 &  &  &  &  &  &  &  &  &  &  &  &  \\ \bottomrule
%\end{tabular}
%
%\end{table}
